UAV-Based Solution for Extending the Lifetime of IoT Devices: Efficiency, Design and Sustainability

Internet of Things (IoT) technology is named as a key ingredient in the evolution towards digitization of many applications and services. A deployment based on battery-powered remote Internet of Things (IoT) devices enables easy installation and operation, yet the autonomy of these devices poses a crucial challenge. A too short lifespan is undesirable from a functional, economical, and ecological point of view. This paper presents a unmanned aerial vehicle (UAV)-based approach to recharge remote Internet of Things (IoT) nodes. An in-depth study of the charging efficiency and optimization of key parameters, and measurements-based verification, is reported on. An actual corresponding design and implementation of the full UAV-based charging system and its proof-of-concept validation are presented. Finally, the sustainability of the proposed solution is discussed. The results presented in this paper hence confirm that the proposed UAV-based approach and design are functionally successful and efficient charging can be achieved, provided the constraints and challenges coming with the approach are adequately dealt with. Moreover, it comes with an overall reduction in ecological footprint for IoT applications relying on battery-powered nodes in need of medium energy and/or considerable lifetime expectation (5 years or more).

==> images/k-analysis/different-receive-coils.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
width=0.8\textwidth,
height=0.3\textwidth,
axis background/.style={fill=gray!10},
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=lightgray204},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={Vertical distance [mm]},
xmajorgrids,
xmin=-8.95, xmax=209.95,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Coupling factor (k) [-]},
ymajorgrids,
ymin=-0.0345544993901741, ymax=0.814542054923342,
ytick style={color=black}
]
\addplot [draw=steelblue31119180, fill=steelblue31119180, forget plot, mark=*, only marks]
table{%
x  y
1 0.147390714
50 0.075932284
100 0.027916606
150 0.011778231
200 0.005789029
};
\addplot [draw=darkorange25512714, fill=darkorange25512714, forget plot, mark=*, only marks]
table{%
x  y
1 0.245296167
50 0.110924996
100 0.04028655
150 0.017253615
200 0.008581866
};
\addplot [draw=forestgreen4416044, fill=forestgreen4416044, forget plot, mark=*, only marks]
table{%
x  y
1 0.396725941
50 0.142531452
100 0.051778514
150 0.0226555
200 0.0114453
};
\addplot [draw=crimson2143940, fill=crimson2143940, forget plot, mark=*, only marks]
table{%
x  y
1 0.775946757
50 0.165203676
100 0.061508011
150 0.027688345
200 0.014255924
};
\addplot [semithick, steelblue31119180]
table {%
1 0.147390714
23.1111111111111 0.113674635720083
45.2222222222222 0.0821730333114235
67.3333333333333 0.0555065729339713
89.4444444444444 0.0352005709914719
111.555555555556 0.0216849941314654
133.666666666667 0.0142944592452872
155.777777777778 0.0112682334680675
177.888888888889 0.00975023417873169
200 0.00578902899999989
};
\addlegendentry{Receive coil dimensions \SI{750}{\milli\meter}}
\addplot [semithick, darkorange25512714]
table {%
1 0.245296167
23.1111111111111 0.176005697185115
45.2222222222222 0.120996257107471
67.3333333333333 0.0795358521088768
89.4444444444444 0.0503708241032136
111.555555555556 0.0317258515764391
133.666666666667 0.0213039495865857
155.777777777778 0.0162864697637606
177.888888888889 0.0133331003101462
200 0.00858186600000005
};
\addlegendentry{Receive coil dimensions \SI{100}{\milli\meter}}
\addplot [semithick, forestgreen4416044]
table {%
1 0.396725941
23.1111111111111 0.252543315357469
45.2222222222222 0.157896504624979
67.3333333333333 0.0986285949312989
89.4444444444444 0.0631085011211098
111.555555555556 0.0422309667550012
133.666666666667 0.0294165641094717
155.777777777778 0.0206116941769313
177.888888888889 0.014288586665698
200 0.0114452999999998
};
\addlegendentry{Receive coil dimensions \SI{1250}{\milli\meter}}
\addplot [semithick, crimson2143940]
table {%
1 0.775946757
23.1111111111111 0.394166081844186
45.2222222222222 0.1921946337485
67.3333333333333 0.101259965328134
89.4444444444444 0.0682887454646447
111.555555555556 0.0559067593059474
133.666666666667 0.0424389082663162
155.777777777778 0.021909210026391
177.888888888889 0.00404079853316752
200 0.0142559240000023
};
\addlegendentry{Receive coil dimensions \SI{1500}{\milli\meter}}
\end{axis}

\end{tikzpicture}

